Zero-Knowledge Proof of Distinct Identity: a Standard-compatible Sybil-resistant Pseudonym Extension for C-ITS

Pseudonyms are widely used in Cooperative Intelligent Transport Systems (C-ITS) to protect the location privacy of vehicles. However, the unlinkability nature of pseudonyms also enables Sybil attacks, where a malicious vehicle can pretend to be multiple vehicles at the same time. In this paper, we propose a novel protocol called zero-knowledge Proof of Distinct Identity (zk-PoDI,) which allows a vehicle to prove that it is not the owner of another pseudonym in the local area, without revealing its actual identity. Zk-PoDI is based on the Diophantine equation and zk-SNARK, and does not rely on any specific pseudonym design or infrastructure assistance. We show that zk-PoDI satisfies all the requirements for a practical Sybil-resistance pseudonym system, and it has low latency, adjustable difficulty, moderate computation overhead, and negligible communication cost. We also discuss the future work of implementing and evaluating zk-PoDI in a realistic city-scale simulation environment.

==> figures/protocol.tex <==
\begin{tikzpicture}[auto, >=latex']
    \node at (1.5,2) {\includesvg[width=50pt]{figures/LEA}};
    \node[rectangle,minimum width =60pt,minimum height =30pt] (0) at (1.5,2) {LEA};
    \node[rectangle,minimum width =50pt,minimum height =30pt] (1) at(0,0) {};
    \node at (0,0) {\includesvg[width=50pt]{figures/alice}};
    \node at (3,0) {\includesvg[width=50pt]{figures/bob}};
    \node at (1.5,-2) {\includesvg[width=50pt]{figures/victor}};
    \node at (-1.5,0) {Alice};
    \node at (4.5,0) [align=center] {Bob\\(Prover)};
    \node at (0,-2) [align=center] {Victor\\(Verifier)};
    \node[rectangle,minimum width =50pt,minimum height =30pt] (2) at(3,0) {};
    \node[rectangle,minimum width =50pt,minimum height =30pt] (3) at(1.5,-2) {};
    \draw[->] (0) --(1);
    \draw[->] (0) --(2);
    \draw[->] (1) --(2);
    \draw[->,>=stealth] (2) --(3);
    \node at (0,1) {$P_a,y_a$};
    \node at (3,1) {$P_b,y_b$};
    \node at (1.5,0.2) {$P_a,y_a$};
    \node at (3.5,-1) {$\pi,P_a,y_a,P_b,y_b$};
    \node at (3.5,2) {\rotatebox{-90}{\resizebox{30pt}{50pt}{\includesvg{figures/wifi}}}};
    \node at (4.8,2) {$\begin{matrix}PF,VF\\pk,vk\end{matrix}$};
\end{tikzpicture}

